HPNet: Deep Primitive Segmentation Using Hybrid Representations

This paper introduces HPNet, a novel deep-learning approach for segmenting a 3D shape represented as a point cloud into primitive patches. The key to deep primitive segmentation is learning a feature representation that can separate points of different primitives. Unlike utilizing a single feature representation, HPNet leverages hybrid representations that combine one learned semantic descriptor, two spectral descriptors derived from predicted geometric parameters, as well as an adjacency matrix that encodes sharp edges. Moreover, instead of merely concatenating the descriptors, HPNet optimally combines hybrid representations by learning combination weights. This weighting module builds on the entropy of input features. The output primitive segmentation is obtained from a mean-shift clustering module. Experimental results on benchmark datasets ANSI and ABCParts show that HPNet leads to significant performance gains from baseline approaches.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

all:  ${PDF} ALLSAMPLES


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES:
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex-dev $(notdir $<)
	cd $(dir $@) && xelatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex-dev $(notdir $<); done

samples/sample-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex-dev $(notdir $<)
	cd $(dir $@) && lualatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex-dev $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut 



clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all docclean
	zip -r $@ acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.*

.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> supp_figures/supp_figure3.tex <==
\begin{figure*}
\centering
\footnotesize
\def\imh{0.073\textwidth}
\def\imw{0.15\textwidth}
\newcommand{\TT}[1]{\raisebox{-0.5\height}{#1}}
\setlength{\tabcolsep}{1pt}
\resizebox{0.95\textwidth}{!}{%
\begin{tabular}{cccccccc}

\rotatebox[origin=c]{90}{G.T} & 
\TT{\includegraphics[width=\imw]   {supp_figures/supp_figure3/31640_gt.png}} & 
\TT{\includegraphics[height=0.11\textwidth]      {supp_figures/supp_figure3/30339_gt.png}} & 
\TT{\includegraphics[width=0.16\textwidth]    {supp_figures/supp_figure3/30410_gt.png}} & 
\TT{\includegraphics[width=0.12\textwidth]    {supp_figures/supp_figure3/31006_gt.png}} & 
\TT{\includegraphics[width=0.13\textwidth]      {supp_figures/supp_figure3/31431_gt.png}} & 
\TT{\includegraphics[width=0.13\textwidth]      {supp_figures/supp_figure3/30276_gt.png}} & 
\TT{\includegraphics[width=\imw]     {supp_figures/supp_figure3/32006_gt.png}} \\

\rotatebox[origin=c]{90}{Ours-nc} & 
\TT{\includegraphics[width=\imw]   {supp_figures/supp_figure3/31640_nc.png}} & 
\TT{\includegraphics[height=0.11\textwidth]      {supp_figures/supp_figure3/30339_nc.png}} & 
\TT{\includegraphics[width=0.14\textwidth]    {supp_figures/supp_figure3/30410_nc.png}} & 
\TT{\includegraphics[width=0.12\textwidth]    {supp_figures/supp_figure3/31006_nc.png}} & 
\TT{\includegraphics[width=0.13\textwidth]      {supp_figures/supp_figure3/31431_nc.png}} & 
\TT{\includegraphics[width=0.13\textwidth]      {supp_figures/supp_figure3/30276_nc.png}} &
\TT{\includegraphics[width=\imw]     {supp_figures/supp_figure3/32006_nc.png}} \\

\rotatebox[origin=c]{90}{Ours-full} & 
\TT{\includegraphics[width=\imw]   {supp_figures/supp_figure3/31640_cc.png}} & 
\TT{\includegraphics[height=0.11\textwidth]      {supp_figures/supp_figure3/30339_cc.png}} & 
\TT{\includegraphics[width=0.145\textwidth]    {supp_figures/supp_figure3/30410_cc.png}} & 
\TT{\includegraphics[width=0.12\textwidth]    {supp_figures/supp_figure3/31006_cc.png}} & 
\TT{\includegraphics[width=0.13\textwidth]      {supp_figures/supp_figure3/31431_cc.png}} & 
\TT{\includegraphics[width=0.13\textwidth]      {supp_figures/supp_figure3/30276_cc.png}} &
\TT{\includegraphics[width=\imw]     {supp_figures/supp_figure3/32006_cc.png}} \\

\end{tabular}
}
\caption{Comparison between our approach without combining the consistency spectral descriptors(`Ours-nc') and our full approach (`Ours-full').}
\label{Figure:Comparison_cc}
\vspace{-0.15in}
\end{figure*}


==> supp_figures/supp_figure4.tex <==
\begin{figure*}
\centering
\footnotesize
\def\imh{0.073\textwidth}
\def\imw{0.15\textwidth}
\newcommand{\TT}[1]{\raisebox{-0.5\height}{#1}}
\setlength{\tabcolsep}{1pt}
\begin{tabular}{cccccccc}

\rotatebox[origin=c]{90}{G.T} & 
\TT{\includegraphics[width=\imw]     {supp_figures/supp_figure4/30071_gt.png}} & 
\TT{\includegraphics[width=\imw]   {supp_figures/supp_figure4/30392_gt.png}} & 
\TT{\includegraphics[height=0.15\textwidth]      {supp_figures/supp_figure4/30506_gt.png}} & 
\TT{\includegraphics[width=0.12\textwidth]    {supp_figures/supp_figure4/31409_gt.png}} & 
\TT{\includegraphics[width=0.09\textwidth]    {supp_figures/supp_figure4/31598_gt.png}} & 
\TT{\includegraphics[width=0.13\textwidth]      {supp_figures/supp_figure4/31697_gt.png}} & 
\TT{\includegraphics[width=0.14\textwidth]      {supp_figures/supp_figure4/31745_gt.png}}  \\

\rotatebox[origin=c]{90}{Ours-ns} & 
\TT{\includegraphics[width=\imw]     {supp_figures/supp_figure4/30071_nc.png}} & 
\TT{\includegraphics[width=\imw]   {supp_figures/supp_figure4/30392_nc.png}} & 
\TT{\includegraphics[height=0.15\textwidth]      {supp_figures/supp_figure4/30506_nc.png}} & 
\TT{\includegraphics[width=0.10\textwidth]    {supp_figures/supp_figure4/31409_nc.png}} & 
\TT{\includegraphics[width=0.085\textwidth]    {supp_figures/supp_figure4/31598_nc.png}} & 
\TT{\includegraphics[width=0.14\textwidth]      {supp_figures/supp_figure4/31697_nc.png}} & 
\TT{\includegraphics[width=0.15\textwidth]      {supp_figures/supp_figure4/31745_nc.png}}  \\

\rotatebox[origin=c]{90}{Ours-full} & 
\TT{\includegraphics[width=\imw]     {supp_figures/supp_figure4/30071_cs.png}} & 
\TT{\includegraphics[width=\imw]   {supp_figures/supp_figure4/30392_cs.png}} & 
\TT{\includegraphics[height=0.15\textwidth]      {supp_figures/supp_figure4/30506_cs.png}} & 
\TT{\includegraphics[width=0.12\textwidth]    {supp_figures/supp_figure4/31409_cs.png}} & 
\TT{\includegraphics[width=0.09\textwidth]    {supp_figures/supp_figure4/31598_cs.png}} & 
\TT{\includegraphics[width=0.13\textwidth]      {supp_figures/supp_figure4/31697_cs.png}} & 
\TT{\includegraphics[width=0.14\textwidth]      {supp_figures/supp_figure4/31745_cs.png}}  \\

\end{tabular}
\caption{Comparison between our approach without combining the smoothness spectral descriptors(`Ours-ns') and our full approach (`Ours-full').}
\label{Figure:Comparison_cs}
\vspace{-0.15in}
\end{figure*}

